MADTP: Multimodal Alignment-Guided Dynamic Token Pruning for Accelerating Vision-Language Transformer

Vision-Language Transformers (VLTs) have shown great success recently, but are meanwhile accompanied by heavy computation costs, where a major reason can be attributed to the large number of visual and language tokens. Existing token pruning research for compressing VLTs mainly follows a single-modality-based scheme yet ignores the critical role of aligning different modalities for guiding the token pruning process, causing the important tokens for one modality to be falsely pruned in another modality branch. Meanwhile, existing VLT pruning works also lack the flexibility to dynamically compress each layer based on different input samples. To this end, we propose a novel framework named Multimodal Alignment-Guided Dynamic Token Pruning (MADTP) for accelerating various VLTs. Specifically, we first introduce a well-designed Multi-modality Alignment Guidance (MAG) module that can align features of the same semantic concept from different modalities, to ensure the pruned tokens are less important for all modalities. We further design a novel Dynamic Token Pruning (DTP) module, which can adaptively adjust the token compression ratio in each layer based on different input instances. Extensive experiments on various benchmarks demonstrate that MADTP significantly reduces the computational complexity of kinds of multimodal models while preserving competitive performance. Notably, when applied to the BLIP model in the NLVR2 dataset, MADTP can reduce the GFLOPs by 80% with less than 4% performance degradation.

==> sec/6_limitation.tex <==
\section{Limitations}
\label{sec:Limitations}
% Our MADTP effectively reduces computational costs in VLTs through token pruning scheme, while preserving the model parameters. 
% The orthogonality of our MADTP with parameter pruning methods has been verified through experimental results provided in Appendix B. Moving forward, our future work focus on integrating parameter pruning scheme into our MADTP framework to achieve comprehensive compression of VLT models, thereby reducing computational and storage requirements.

%Our MADTP significantly reduces computational costs in VLTs through token pruning scheme, while preserving the model parameters. Experimental results in Appendix C confirm the compatibility of MADTP with parameter pruning methods. Our future work involves integrating a parameter pruning scheme into the MADTP framework for comprehensive VLT model compression.
%, reducing computational and storage requirements.

